Rich Screen Reader Experiences for Accessible Data Visualization

Current web accessibility guidelines ask visualization designers to support screen readers via basic non-visual alternatives like textual descriptions and access to raw data tables. But charts do more than summarize data or reproduce tables; they afford interactive data exploration at varying levels of granularity -- from fine-grained datum-by-datum reading to skimming and surfacing high-level trends. In response to the lack of comparable non-visual affordances, we present a set of rich screen reader experiences for accessible data visualization and exploration. Through an iterative co-design process, we identify three key design dimensions for expressive screen reader accessibility: structure, or how chart entities should be organized for a screen reader to traverse; navigation, or the structural, spatial, and targeted operations a user might perform to step through the structure; and, description, or the semantic content, composition, and verbosity of the screen reader's narration. We operationalize these dimensions to prototype screen-reader-accessible visualizations that cover a diverse range of chart types and combinations of our design dimensions. We evaluate a subset of these prototypes in a mixed-methods study with 13 blind and low vision readers. Our findings demonstrate that these designs help users conceptualize data spatially, selectively attend to data of interest at different levels of granularity, and experience control and agency over their data analysis process. An accessible HTML version of this paper is available at: http://vis.csail.mit.edu/pubs/rich-screen-reader-vis-experiences.

==> tables/_likert-ratings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Likert-Ratings Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bgroup
\begin{table*}[]
\caption{
Likert-ratings for each prototype: Table, Multi-View, and Targeted.
Participants selected responses on the linear scale: \emph{[1 = Very Difficult (Very Unenjoyable), 5 = Very Easy (Very Enjoyable)]}.
% \hl{TODO: Fill in numbers when Eval is complete. Identify and indicate statistically significant rating differences between the Prototypes (if any).} // CRYSTAL: I think our sample size is too small to really run any t-tests for statistical significance. 
}

\centering
\small
\def\arraystretch{1.1}

\begin{tabular}{m{7cm} m{1.5cm} c{2.2cm} c{2.2cm} c{2.2cm}}
\hline
\textsc{question} : \emph{When using this prototype ...}
& \textsc{task}~\cite{brehmer_multi-level_2013}
% & \textsc{scale}
& \textsc{table} 
& \textsc{multi-view}
& \textsc{targeted}
\\
\hline\hline

\rowcolor{anti-flashwhite}
% After understanding how this Prototype works, how enjoyable was it to interact with the data?
% How enjoyable was it to interact with the data using this Prototype?
\emph{How enjoyable was it to interact with the data?}
& \texttt{enjoy}
% & [1=Unenjoyable, 5=Enjoyable]
& $\mu=3.31$, $\sigma=0.95$
& $\mu=3.77$, $\sigma=1.01$
& $\mu=3.54$, $\sigma=0.97$
\\

% After understanding how this Prototype works, how easy was it to generate and answer questions about the data?
% How easy was it to generate and answer questions about the data using this Prototype?
\emph{How easy was it to generate and answer questions?}
& \texttt{discover}
% & [1=Difficult, 5=Easy]
& $\mu=3.15$, $\sigma=1.34$
& $\mu=3.00$, $\sigma=1.08$
& $\mu=3.23$, $\sigma=1.17$
\\

\rowcolor{anti-flashwhite}
% If you already knew what information you were trying to find, how easy would it be to look up or locate those data points using this Prototype?
\emph{If you already knew what information you were trying to find, how easy would it be to look up or locate those data?}
& \texttt{lookup}, \texttt{locate}
% & [1=Difficult, 5=Easy]
& $\mu=3.31$, $\sigma=1.32$
& $\mu=3.77$, $\sigma=1.17$
& $\mu=3.38$, $\sigma=1.19$
\\

% If you didn't already know which information you were trying to find, how easy would it be to browse or explore the data using the this Prototype?
\emph{If you didn't already know which information you were trying to find, how easy would it be to browse or explore the data?}
& \texttt{browse}, \texttt{explore}
% & [1=Difficult, 5=Easy]
& $\mu=3.00$, $\sigma=1.68$
& $\mu=2.69$, $\sigma=1.11$
& $\mu=3.00$, $\sigma=1.29$
\\

\hline
% \textsc{question}
% & \textsc{aspect}
% % & \textsc{scale}
% & \textsc{data table} 
% & \textsc{multi-view}
% & \textsc{random access}
% \\
% \hline

\rowcolor{anti-flashwhite}
% How easy was it to learn to use this Prototype?
\emph{How easy was it to learn to use?}
& Learnability
% & [1=Difficult, 5=Easy]
& $\mu=4.15$, $\sigma=0.99$
& $\mu=2.69$, $\sigma=0.75$
& $\mu=3.15$, $\sigma=1.34$
\\

% When interacting with data, how useful would it be to have access to the style of interaction presented in this Prototype?
\emph{How useful would it be to have access to this interaction style for engaging with data?}
& Usability, Acceptance
% & [1=Difficult, 5=Easy]
& $\mu=4.15$, $\sigma=0.80$
& $\mu=4.00$, $\sigma=0.82$
& $\mu=4.15$, $\sigma=1.07$
\\

\hline
\end{tabular}
\label{table:likert-ratings}
\vspace{-5mm}
\end{table*}
\egroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

